Taiwan Axion Search Experiment with Haloscope: Designs and operations

We report on a holoscope axion search experiment near $19.6\ {\rm \mu eV}$ from the TASEH collaboration. The experiment is carried out via a frequency-tunable cavity detector with a volume $V = 0.234\ {\rm liter}$ in a magnetic field $B_0 = 8\ {\rm T}$. With a signal receiver that has a system noise temperature $T_{\rm sys} \cong 2.2\ {\rm K}$ and experiment time about 1 month, the search excludes values of the axion-photon coupling constant $g_{\rm a\gamma\gamma} \gtrsim 8.1 \times 10^{-14} \ {\rm GeV}^{-1}$, a factor of 11 above the KSVZ model, at the 95\% confidence level in the mass range of $19.4687-19.8436\ {\rm \mu eV}$. We present the experimental setup and procedures to accomplish this search.

==> full_author.tex <==
%Hsin Chang
\author{Hsin~Chang}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan}
%Jing-Yang Chang
\author{Jing-Yang~Chang}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan} 
%Yi-Chieh Chang
\author{Yi-Chieh~Chang}\affiliation{National Synchrotron Radiation Research Center, Hsinchu 30076, Taiwan} 
%Yu-Han Chang
\author{Yu-Han~Chang}\affiliation{Department of Physics, National Chung Hsing University, Taichung City 402, Taiwan}
%Yuan-Hann Chang
\author{Yuan-Hann~Chang}\affiliation{Institute of Physics, Academia Sinica, Taipei City 115201, Taiwan}
\affiliation{Center for High Energy and High Field Physics, National Central University, Taoyuan City 32001, Taiwan}
%Chien-Han CHen
\author{Chien-Han~Chen}\affiliation{Institute of Physics, Academia Sinica, Taipei City 115201, Taiwan} 
%Ching-Fang Chen 
\author{Ching-Fang~Chen}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan}
%Kuan-Yu CHen
\author{Kuan-Yu~Chen}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan} 
%Yung-Fu Chen
\author{Yung-Fu~Chen}
\email[Correspondence to: ]{yfuchen@ncu.edu.tw}
\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan} 
%Wei-Yuan James Chiang
\author{Wei-Yuan~Chiang}\affiliation{National Synchrotron Radiation Research Center, Hsinchu 30076, Taiwan}
%Wei-Chen Chien
\author{Wei-Chen~Chien}\affiliation{Department of Physics, National Chung Hsing University, Taichung City 402, Taiwan}
%Hien Thi Doan
\author{Hien~Thi~Doan}\affiliation{Institute of Physics, Academia Sinica, Taipei City 115201, Taiwan} 
%Wei-Cheng Hung
\author{Wei-Cheng~Hung}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan} 
%Watson Kuo
\author{Watson~Kuo}\affiliation{Department of Physics, National Chung Hsing University, Taichung City 402, Taiwan} 
%Shou-Bai Lai
\author{Shou-Bai~Lai}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan} 
%Han-Wen Liu
\author{Han-Wen~Liu}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan} 
%Min-Wei Ouyang
\author{Min-Wei~OuYang}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan}
%Ping-I Wu
\author{Ping-I~Wu}\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan} 
%Shin-Shan Yu
\author{Shin-Shan~Yu}
%\email[Correspondence to: ]{syu@phy.ncu.edu.tw}
\affiliation{Department of Physics, National Central University, Taoyuan City 32001, Taiwan}
\affiliation{Center for High Energy and High Field Physics, National Central University, Taoyuan City 32001, Taiwan}


\collaboration{TASEH Collaboration}%\noaffiliation



